Avatar Knowledge Distillation: Self-ensemble Teacher Paradigm with Uncertainty

Knowledge distillation is an effective paradigm for boosting the performance of pocket-size model, especially when multiple teacher models are available, the student would break the upper limit again. However, it is not economical to train diverse teacher models for the disposable distillation. In this paper, we introduce a new concept dubbed Avatars for distillation, which are the inference ensemble models derived from the teacher. Concretely, (1) For each iteration of distillation training, various Avatars are generated by a perturbation transformation. We validate that Avatars own higher upper limit of working capacity and teaching ability, aiding the student model in learning diverse and receptive knowledge perspectives from the teacher model. (2) During the distillation, we propose an uncertainty-aware factor from the variance of statistical differences between the vanilla teacher and Avatars, to adjust Avatars' contribution on knowledge transfer adaptively. Avatar Knowledge Distillation AKD is fundamentally different from existing methods and refines with the innovative view of unequal training. Comprehensive experiments demonstrate the effectiveness of our Avatars mechanism, which polishes up the state-of-the-art distillation methods for dense prediction without more extra computational cost. The AKD brings at most 0.7 AP gains on COCO 2017 for Object Detection and 1.83 mIoU gains on Cityscapes for Semantic Segmentation, respectively. Code is available at https://github.com/Gumpest/AvatarKD.

==> table/ensemble.tex <==
\begin{table}[h]
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{3mm}
	\centering
	\caption{\textbf{Experiment on the performance of ensemble separations on COCO dataset with RetinaNet-X101.} The weighted box fusion method (WBF) is adopted for ensemble.}
    
    \label{tab:multi-tea}
	\begin{tabular}{c|cccc}
	\shline
    \multirow{2}*{Vanilla Teacher} & \multicolumn{4}{c}{Separations Ensemble} \\
    \cline{2-5}
    ~ & 2 & 4 & 6 & 8\\
    \shline
	41.2 & 41.2 & 41.3 & \textbf{41.4} & \textbf{41.4} \\
    \shline
	\end{tabular}
	% \vspace{-2mm}
\end{table}
